First-principles modelling of the magnetic structure of the lightest nuclear systems using effective field theory without pions

The strong interaction, i.e., quantum chromodynamics at the low energy nuclear regime, is notoriously known to be challenging for predictive modeling. Here, we use the simplest possible nuclear effective field theory (EFT), and show that in the case of the magnetic structure of nuclear systems with $A=2$ and $A=3$ nucleons, it is highly precise as well as predictive. The theoretical framework is the pionless EFT (\pilesseft), of point nucleons with contact interactions, expanded consistently up to next-to-leading order (NLO) in perturbation theory, i.e., including only eleven low-energy parameters, and augmented by a novel Bayesian analysis of theoretical uncertainties. The theory accurately predicts the shell structure reflected in the values of the magnetic moments and reactions of these nuclei within $\approx 1\%$ calculated theoretical uncertainty. We show that this perfect prediction originates in implicit a-posteriori properties of the calculation, particularly an unexpectedly small expansion parameter, as well as a vanishing contribution from the two-body isoscalar current.

==> Bayesian_approach2.tex <==
In the following, we expand upon the approach we used  to evaluate the truncation uncertainty and the size of the expansion parameter of a set of observables whose expansion is $\langle{M_1}\rangle=\langle{M_1}\rangle_{\text LO} \cdot \left ( 1+c^{\text NLO}_{M_1} \delta + c^{\text N2LO}_{M_1} \delta^2+{\mathcal{O}} (\delta^3)\right)$.

\subsection{The Bayesian probability distribution of the expansion parameter}
We use information theory arguments to understand the expected behaviour of the expansion convergence rate. The ratio of the k$^{th}$ and l$^{th}$ expansion terms should be proportional to $\delta^{k-l}$ ($\delta$ is the expansion parameter), \textit{i.e.}, 
\begin{equation}
r_{k-l}^{M_1}\delta^{k-l}\equiv\left|\frac{c^{{\text {N}}^k\text{LO}}_{M_1}}{c^{{\text {N}}^l\text{LO}}_{M_1}}\right|.
\end{equation}
\pilesseft formalism suggests that $r_{k-l}^{M_1}$  should be a natural number. We interpret this as a statement regarding the nature of the distribution of these numbers. In layman's terms, one would be surprised if these numbers deviate much from 1. In other words, these coefficients have some natural range of change $\frac{1}{\alpha} < r_{k-l}^{M_1} < \alpha$, where $\alpha$ is a measure of naturalness. One can expect $\alpha$ a factor of 2-3, while bigger variations are acceptable as long as they are rare. From a Bayesian point of view, $r_{k-l}^{M_1}$ are independent and identically distributed random variables (i.i.d) with an average of about $1$ and their logarithm has a (unknown) standard deviation of $\log \alpha$. 

Information theory now states that the probability density function (pdf) $f(r)$ should maximize the entropy $S[f]=-\int dr f(r)\log f(r)$ subject to the constraints $\overline{\log r} =0$ and $\overline{ (\log r-\overline{\log r})^2}=\log \alpha$.
Thus, the log-average of $r_{k-l}^{M_1}\delta^{k-l}$ should be the expansion parameter $(k-l)\log{\delta}$. These lead to a pdf $f(r)$ that is a log-normal distribution.

One can now use a sample of the size $n$ to estimate the expansion parameter, i.e., $\overline{\log{\delta}}=\frac{1}{n}\sum_{i=1}^n \frac{1}{k-l} \log\left( r_{k-l}^{M_1(i)}\delta^{k-l}\right) $. Then, by using Bayes theorem, the resulting distribution for the expansion parameter is Student's {\it t}-distribution with n-1 degrees of freedom $\frac{\log\delta-\overline{\log{\delta}}}{\overline{\sigma^2}/\sqrt{n}}\sim T (\overline{\sigma^2}, n-1)$. 

\subsection{The Bayesian probability distribution of the truncation error of an expansion, given a prior for the expansion parameter}

A good estimate for the truncation error is the maximal coefficient in an expansion of order $k$, multiplied by $\delta^{k+1}$. In Refs.~\cite{Griesshammer:2015ahu, PhysRevC.92.024005, Cacciari2011}, a Bayesian probability distribution is calculated for the truncation error under the assumption of a natural expansion, albeit in the case where the expansion parameter $\delta$ is known. In what follows, we combine their idea with the probability distribution for the expansion parameter found above, to find the Bayesian probability distribution that the NLO result will deviate by $\Delta$ from the true value. Then, 
\begin{align}\label{eq_delta}
\nonumber
&pr\left (\Delta \big | \left\{a^{\text NLO}_{M^k_1}\right\}_{k=1}^n\right)=\\
&\int d\delta pr\left (\Delta \big | \left\{c^{\text NLO}_{M^k_1}\right\}_{k=1}^n, \delta\right)\cdot pr\left (\delta \big | \left\{a^{\text NLO}_{M^k_1}\right\}_{k=1}^n\right).
\end{align}
$pr (\Delta \big | \left\{c^{\text NLO}_{M^k_1}\right\}_{k=1}^n, \delta)$ is calculated in~Ref.~\cite{Griesshammer:2015ahu}, and at NLO, is roughly constant for $|\Delta|\le R_\xi (\delta)$, and decays as $1/|\Delta|^3$ for $|\Delta|\ge R_\xi (\delta)$, where $R_\xi (\delta)=max\left (1, \left\{c^{\text NLO}_{M^k_1}\right\}_{n=1}\right)\delta^2$. The exact functional form depends on the prior assumption for $\left\{c^{\text NLO}_{M^k_1}\right\}_{k=1}^n$, but a common behavior of all the checked priors is that at a degree of belief of $\frac{k}{k+1}$ (translating to $\approx 67\%$ for NLO calculations) the resulting truncation error is less than $R_\xi (\delta) \delta^{k+1}$. 

As the pdf for $\delta$, we take the Student's {\it t}-distribution found in the previous subsection.

